Continuous reasoning for adaptive container image distribution in the cloud-edge continuum

Cloud-edge computing requires applications to operate across diverse infrastructures, often triggered by cyber-physical events. Containers offer a lightweight deployment option but pulling images from central repositories can cause delays. This article presents a novel declarative approach and open-source prototype for replicating container images across the cloud-edge continuum. Considering resource availability, network QoS, and storage costs, we leverage logic programming to (i) determine optimal initial placements via Answer Set Programming (ASP) and (ii) adapt placements using Prolog-based continuous reasoning. We evaluate our solution through simulations, showcasing how combining ASP and Prolog continuous reasoning can balance cost optimisation and prompt decision-making in placement adaptation at increasing infrastructure sizes.

==> img/asp_workflow.tex <==
% \begin{figure}
% \centering
% \resizebox{0.47\textwidth}{!}{%
% \begin{tikzpicture}[node distance=2cm]
%     \node(modeling) at (0,1) {Modeling};
%     \node(modeling) at (4,1) {Solving};
%     \node(modeling) at (8,1) {Interpreting};

%     \node(problem) [wf_node] at (0,0) {Problem};
%     \node(d0) [above left of=problem] {};
%     % \node(lp) [wf_node, below of=problem] {Logic Program};
%     \node(lp) [wf_node] at (0,-2) {Logic Program};
%     \node(d1) [below right of=lp] {};
%     \draw [arrow] (problem) -- (lp);

%     \node(between_lp_solver) at (2,-2) {};
%     \node(between_problem_grounder) at (2,0) {};
%     \draw [thick] (between_lp_solver) |- (between_problem_grounder);
%     \draw [thick] (between_lp_solver) -| (between_problem_grounder);
%     \draw [thick] (lp) -| (between_lp_solver);
    
    
%     \node(grounder) [wf_node] at (4,0) {Grounder};
%     \node(d_grounder) [above left of=grounder] {};
%     % \node(lp) [wf_node, below of=problem] {Logic Program};
%     \node(solver) [wf_node] at (4,-2) {Solver};
%     \node(d_solver) [below right of=solver] {};
%     \draw [arrow] (grounder) -- (solver);
%     \draw [arrow] (between_problem_grounder) |- (grounder);
%     % \draw [] (grounder) -- (between_problem_grounder);

%     \node(between_solver_solution) at (6,-2) {};
%     \node(between_grounder_as) at (6,0) {};
%     \draw [thick] (between_solver_solution) |- (between_grounder_as);
%     \draw [thick] (between_solver_solution) -| (between_grounder_as);
%     \draw [thick] (solver) -| (between_solver_solution);
    

%     \node(answer_sets) [wf_node] at (8,0) {Answer sets};
%     \node(d_answer_sets) [above left of=answer_sets] {};
%     % \node(lp) [wf_node, below of=problem] {Logic Program};
%     \node(solution) [wf_node] at (8,-2) {Solution};
%     \node(d_solution) [below right of=solution] {};
%     \draw [arrow] (answer_sets) -- (solution);
%     \draw [arrow] (between_grounder_as) |- (answer_sets);
    
%     \begin{pgfonlayer}{background}
%         \path[rounded corners, draw=black!50, dashed] (d0) rectangle (d1);
%         \path[rounded corners, draw=black!50, dashed] (d_grounder) rectangle (d_solver);
%         \path[rounded corners, draw=black!50, dashed] (d_answer_sets) rectangle (d_solution);
%         % \path (dummy_dec.south -| dummy_dec.east)+(+0.5,-0.3) node (b) {};
%         % \path (-2,-2)--(2,2) node (c) {};
          
%         % \path[fill=yellow!20,rounded corners, draw=black!50, dashed]
%             % (a) rectangle (c);           
%         % \path (waitNo.north west)+(-0.2,0.2) node (a) {};
%     \end{pgfonlayer}
% \end{tikzpicture}
% }
% \caption{The typical ASP workflow.}
% \label{asp:workflow}
% \end{figure}


==> src/old_preliminaries.tex <==
% Ciao Damiano, ho iniziato ad abbozzare la sezione, se ci sono cazzate/la organizzeresti diversamente cancella pure
\section{Preliminaries: Logic Programming, Prolog, \& ASP}
\label{sec:preliminaries}
In this section, we provide some background on Logic Programming~\cite{Lloyd87},  the Prolog programming language~\cite{sterling1994art}, and Answer Set Programming (ASP)~\cite{brewka2011asp}, which is needed to then fully understand the next sections.

\subsection{Logic Programming}
\label{subsec:lp}
We consider a logic program as s set of \textit{normal rules} (also called \textit{clauses}) of the form:
$$
h \impl b_1, \dots, b_n
$$
where $h$ is an atom and the $b_i$ are literals (atoms or negated atoms).
An example of an atom is $edge(a,b)$.
We use the standard notation $name/arity$ (called functor) to compactly represent a set of atoms or clauses with head the atom with name $name$ and $arity$ arguments.
That is, for the previous atom we write $edge/2$.
The atom $h$ is called \textit{head} while the conjunction of the literal $b_i$ is called \textit{body}.
% For a rule $r$ we use  and $B(r)$ to denote, respectively, its head and its body.
The meaning is that, if all the literals in the body are true, $h$ is true.
If the head is empty, the rule is called \textit{constraint}, while if the body is empty, the rule is called \textit{fact} (and the neck operator, $\impl$, is omitted).
Rules are often also called \textit{clauses}.
A \textit{predicate} is a set of clauses with the same functor.
A rule without variables is called \textit{ground}.
The \textit{substitution} is the process of replacing variables with constants, and if it grounds all the variables it is called \textit{grounding}.
Lastly, \textit{unification} aims to check whether the rules can be made syntactically equal by applying a set of substitutions.

\subsection{Prolog}
\label{subsec:prolog}
Prolog~\cite{Lloyd87,DBLP:series/lncs/Warren23} is a logic programming language as it is based on first-order logic~\cite{Lloyd87}.
A Prolog program is a finite set of normal rules.
% \textit{clauses} of the form:
% %
% \begin{code}
% a :- b1, ... , bn.
% \end{code}
% \vspace{-1.75mm}
% %
% \noindent 
% \stefano{stating that $a$ holds when {\tt b1} $\wedge\ \cdots\ \wedge$ {\tt bn} holds, where {\tt n}$\geq$0 and {\tt a}, {\tt b1}, ..., {\tt bn} are literals.
% Clauses can also contain inclusive disjunctions (i.e. logic ORs) among literals {\tt\small bi} and {\tt\small bj}, represented by {\tt\small bi; bj}.
% Clauses with empty condition are called \textit{facts}.
Prolog variables begin with upper-case letters (except for the anonymous variable, that is represented with an underscore, $\_)$, lists are denoted by square brackets, and negation by $\backslash +$.

Prolog programs can be queried, and the Prolog interpreter tries to answer each query by applying a process called \textit{resolution} (SLDNF~\cite{DBLP:conf/adbt/Clark77}): the resolution starts with a \textit{query} (conjunction of atoms), also called \textit{goal}, that we denote by prepending \textit{?-} to the atoms to prove.
Then, iteratively, it selects a subgoal and replaces it with the body of a clause in the program which has the head unifiable with it.
If, in a certain iteration, the (sub)goal is empty, the query succeeds; otherwise, if there are no more clauses that can be unified with the selected (sub)goal, the query fails.
The resolution is sound and complete.
However, Prolog implementations, such as SWI-Prolog~\cite{wielemaker2012swi}, adopt a non-complete resolution, since the first clause (in order of appearance in the program) that unifies with the considered subgoal is always selected: this can generates an infinite derivation.
Queries can also contain variables.
If so, the variables are replaced with the constant that makes the query true.
Prolog adopts negation as failure: if, during the derivation, a negative literal is encountered (denoted with the symbol $\backslash +$), the Prolog engine tries to prove its positive version.
If this proof fails, the negated version of it succeeds, and the derivation continues.
An important point is that negated literals must be ground when proving it, to avoid the problem of floundering~\cite{sterling1994art}.

To clarify, consider Example~\ref{ex:running_prolog}.
\begin{example}[Path]
\label{ex:running_prolog}
The following well-known example models the search of a path in a graph:
\begin{code}
edge(a,b).
edge(b,d).
edge(a,c).
edge(c,d).
path(X,Y):- edge(X,Y).
path(X,Y):- edge(X,Z), path(Z,Y).
\end{code}
The first four facts state that there are directed edges that connect nodes $a$ and $b$, $b$ and $c$, and $a$ and $d$.
The fifth line contains a rule stating that there is a path between two nodes $X$ and $Y$ if there is an edge that connects them.
The last rule states that there is a path between two nodes $X$ and $Y$ if there is an intermediate node $Z$ from which there is a path towards $Y$.
We may be interested in checking whether a path between nodes $a$ and $d$ exist.
To do so, we can ask the query $?- path(a,d)$, and we get two succeeding solutions.
If we ask the query $?- path(a,X)$, we get as solutions all the substitutions to $X$ that make the query true, namely $X = b$, $X = c$, $X = d$, and $X = d$.
Note that $X = d$ is reported twice, since, for this example, there are two paths from $a$ to $d$.
\end{example}

\subsection{Answer Set Programming}
\label{subsec:ASP}

Answer Set Programming (ASP)~\cite{brewka2011asp} is a declarative knowledge representation formalism rooted in the stable model semantics of logic programs~\cite{gelfond1988stable}, particular efficient in modelling and solving combinatorial and optimisation problems (despite being not Turing complete).
% , that can be used to model and solve problems up to $\Sigma_2^P$ in the polynomial hierarchy.
% It has been successfully applied in many domains, ranging from a variety of industrial problems to ... .
% In ASP, problems are encoded by means of \emph{logic programs}, whose ``solutions'' can be interpreted back onto solutions of the original problem. 
% Thus, users do not have to describe \emph{how} to compute solutions, but \emph{what} are the solutions.
% In this section, we recap the basics of ASP.
% The interested reader can refer to ... for a full reference on the last standardization of the language, and to ... for an introduction to its modeling features.
% In the rest of the paper, we will refer to the \textsc{GrinGo} input language.

An answer set program is a set of disjunctive rules.
As usual, we only consider \textit{safe} rules, i.e., rules where each variable appears at least once in a positive literal.
Modern answer set solvers such as clingo~\cite{gebser2019clingo}, introduce many syntactic shortcuts, which ease the modeling task.
We briefly introduce the ones that are relevant to our encodings.
A \emph{choice rule} is an expression
$$
L\ \{h_1; \dots; h_m\} \ U \impl b_1, \dots, b_n
$$
where each $h_i$ is an atom, each $b_j$ is a literal, and $L$ and $U$ are integers with $L \leq U$.
$L$ and $U$ can be omitted: in this case, by default, $L = 0$ and $U$ is equal to the number of atoms $h_m$.
\damiano{nell'esempio del graph coloring usiamo i : e nel programma anche tuple di atomi, bisogna specificare qua}
An \emph{integrity constraint} is an expression:
$$
\impl b_1, \dots, b_n
$$
where each $b_i$ is a literal.
% An integrity ensures no answer sets can exist where the conjunction of $b_i$ is true.
A \emph{weak constraint} is an expression
$$
\wc b_1, \dots, b_n [C@L,X]
$$
where $C$ is a variable or an integer called \textit{cost} (or \textit{weight}), $L$ is an integer called \textit{priority level} $L$, and $X$ is a tuple of atoms \damiano{that can be omitted if the weak constraint is ground}.
% aggregati non vengono usati
\emph{Aggregates}~\cite{alviano2018aggregates} are set functions over sets of terms with the syntax 
$$
k_1 \ c_1 \ \# \varphi \{\epsilon_0 : l_0; \dots ; \epsilon_n : l_n\} \ c_2 \ k_2
$$
where $k_1$ and $k_2$ are integer constants, $c_1$ and $c_2$ are arithmetic comparison operators, $\varphi$ is an aggregate function symbol such as \texttt{\#max}, \texttt{\#sum}, \texttt{\#count}, and the $\epsilon_i : l_i$ are tuples of terms and literals.
% An example of aggregate atom is \texttt{\#count\{A : p(A)\} = 2}, that is true if the number of ground substitutions for $A$ that make $p(A)$ true is $2$.
% Examples over arithmetic terms are \texttt{\#max}, \texttt{\#sum}, \texttt{\#count}.
% \damiano{mettere esempio come per cr e ic}
% \atterms are not a language extension, but a specific feature of the \clingo system that we adopt in this paper for the experimental evaluation.
% \damiano{lo diciamo anche sotto}
% Other ASP systems support similar features under a different name.
% \texttt{@}-terms are special terms, whose function name starts with the character \texttt{@} that are replaced with the output of a user-defined procedure upon grounding time.
% We will use \texttt{@}-terms to perform (fixed precision) floating point arithmetic since ASP does not natively support it.
% Example~\ref{ex:running_asp} shows an example of an answer set program.

The semantics of Answer Set Programming is based on the concept of stable model~\cite{gelfond1988stable}.
To define it, we need some additional notions.
An interpretation $\mathcal{I}$ is a set of atoms.
An interpretation $\mathcal{I}$ \emph{satisfies} a rule $\rho$ if $\mathcal{I} \subseteq B^{+}(\rho)$ and $\mathcal{I} \cap B^{-}(\rho) = \{\}$, where $B^{+}(\rho)$ and $B^{-}(\rho)$ are the set of positive and negative literals in the body of $\rho$, respectively.
If an interpretation $\mathcal{I}$ satisfies all the rules in $\rho \in P$, $\mathcal{I}$ is a \emph{model} of $P$.
The \emph{reduct} of $P$ w.r.t. $\mathcal{I}$, denoted as $P^{\mathcal{I}}$, is the logic program we obtain by (i) removing all rules $\rho \in P$ such that $B^{+}(\rho) \not\subseteq \mathcal{I}$ and (ii) removing from the body of each rule $\rho \in P$ the literals $B^{-}(\rho) \cup \mathcal{I}$.
An interpretation $\mathcal{I}$ is a \emph{stable model} (or \emph{answer set}) of the logic program $P$ if $\mathcal{I}$ is a subset-minimal model of $P^{\mathcal{I}}$.
ASP semantics is fully declarative and the order of rules within the program and order of literals within the rules' body does not alter it.

A choice rule, as a standalone logic program, generates an answer set for each subset of the atoms in the head of size at least $L$ and at most $U$, whenever the body is true.
If we introduce weak constraints into an answer set program, an answer set is \emph{optimal} whenever it minimizes its cost in a decreasing fashion level-wise.
\damiano{la semantica per gli aggregati è complicata, non credo dobbiamo metterla qui, ma sicuramente serve acennare qualcosa}

We denote the set of answer sets of a logic program $P$ by $AS(P)$.
Logic programs under the stable model semantics might admit none, one, or more answer sets.
We say that a logic program is \emph{incoherent} if it admits no answer sets, \emph{coherent} otherwise.
To clarify the syntax and the semantics of ASP, consider the following examples.


% A choice rule, as a standalone logic program, generates an answer set for each subset of $\{a_1, \dots, a_k\}$ of size at least $L$ and at most $K$, whenever $B$ is true.

% \subsection{Syntax}
% \antonio{\noindent Let $\mathcal{C}, \mathcal{V}, \mathcal{F}, \mathcal{P}$ be finite disjoint sets of \emph{constants}, \emph{variables}, \emph{function names} and \emph{predicate names}. The \emph{arity} of a function, predicate name is an integer denoted by $\sigma(p)$, for each $p \in \mathcal{F} \cup \mathcal{P}$. A \emph{term} is either a constant, a variable or an expression $f(t_1, \dots, t_k)$ where $f \in \mathcal{F}, \sigma(f) = k$ and $t_i$ is a term. An \emph{atom} is an expression $p(t_1, \dots, t_k)$ where $p \in \mathcal{P}, \sigma(p) = k$ and $t_i$ is a term.
% \noindent A \emph{(normal) logic program} is a set of \emph{rules}, a rule $\rho$ is an expression:
% $$h \leftarrow a_1, \dots, a_k, \lnot b_1, \dots, \lnot b_m$$
% \noindent where $a_i, b_i$ are atoms. We denote $H(\rho) = h$ as the \emph{head} of the rule, $B(\rho)$ as the \emph{body} of the rule, which can be partitioned into $B^{+}(\rho) = \{a_1, \dots, a_k\}$ and $B^{-}(\rho) = \{b_1, \dots, b_m\}$. The symbol $\lnot$ denotes \emph{negation-as-failure}. A \emph{literal} is either an atom or a negated atom, and we say the literals $a, \lnot a$ are \emph{opposite literals}.}

% \subsection{Semantics}
% \antonio{\noindent Let $P$ be a logic program without variables. A logic program with variables is regarded as syntactic sugar for its variable-less counterpart. The \emph{grounding process} maps a program with variables into a propositional program. An interpretation $\mathcal{I}$ is a set of atoms. An interpretation $\mathcal{I}$ \emph{satisfies} a rule $\rho$ if $\mathcal{I} \subseteq B^{+}(\rho)$ and $\mathcal{I} \cap B^{-}(\rho) = \{\}$. If an interpretation $\mathcal{I}$ satisfies all the rules in $\rho \in P$, $\mathcal{I}$ is a \emph{model} of $P$. The \emph{reduct} of $P$ wrt $\mathcal{I}$, denoted as $P^{\mathcal{I}}$ is the logic program we obtain by (i) removing all rules $\rho \in P$ such that $B^{+}(\rho) \not\subseteq \mathcal{I}$ and (ii) removing from the body of each rule $\rho \in P$ the literals $B^{-}(\rho) \cup \mathcal{I}$. An interpretation $\mathcal{I}$ is a \emph{stable model} (or \emph{answer set}) of the logic program $P$ if $\mathcal{I}$ is a subset-minimal model of $P^{\mathcal{I}}$.
% We denote the set of answer sets of a logic program $P$ by $AS(P)$. Notice logic programs under the stable model semantics might admit none, one or more answer sets. We say a logic program is \emph{incoherent} if it admits no answer sets, \emph{coherent} otherwise.}
%
% TODO: Merge syntactic sugar + modeling in un'unica sezione, prendere 3-coloring dall'inizio, aggiungere una regola alla volta e mostrare come cambiano gli answer set. Questo secondo me allegerisce la presentazione.
% \subsection{Syntactic sugar}


% \paragraph{Choice rules.}\antonio{A \emph{choice rule} is an expression $$L\ \{a_1; \dots, a_k\} \ U \leftarrow B$$ where $B$ is a conjunction of literals (as in normal rule's body) and $L, U$ are integers with $L \le U$. A choice rule, as a standalone logic program, generates an answer set for each subset of $\{a_1, \dots, a_k\}$ of size at least $L$ and at most $K$, whenever $B$ is true.}

\begin{example}[Choice Rule]
\label{ex:choice_rule}
The following logic program:
\begin{code}
1 {a; b; c} 2.
\end{code}
Admits six answer sets: $\{a, b\}, \{b, c\}, \{a, c\}, \{a\}, \{b\}$, and $\{c\}$.
\end{example}

% \paragraph{Integrity constraints} \antonio{\noindent An \emph{integrity constraint} is an expression: $$\leftarrow B$$ where $B$ is a conjunction of literals. An integrity ensures no answer sets can exist where $B$ is true.}

\begin{example}[Choice Rule and Integrity Constraint]
\label{ex:choice_rule_and_constraint}
The following logic program extends Example~\ref{ex:choice_rule} with an integrity constraint:
\begin{code}
1 {a; b; c} 2.
:- a.
\end{code}
It admits three answer sets: $\{b, c\}$ and $\{b\}, \{c\}$.
The constraint cuts the three answer sets of Example~\ref{ex:choice_rule} with $a$ included.
\end{example}

% \paragraph{Weak constraints} \antonio{\noindent A \emph{weak constraint} is an expression: 
% $$\leftarrow B [C@L,X]$$
% that assigns to answer sets where $B$ is true a \emph{cost} $C$ at \emph{priority level} $L$ for each distinct tuple $X$. An answer set is \emph{optimal} whenever it minimizes its cost in a decreasing fashion level-wise.}
\begin{example}[Choice Rule, Integrity Constraint, and Aggregate]
\label{ex:choice_rule_ic_and_agg}
The following logic program extends Example~\ref{ex:choice_rule_and_constraint} with an aggregate:
\begin{code}
1 {a; b; c} 2.
:- a.
s(X):- X = #sum{1 : b; 2 : c}.
\end{code}
It admits three answer sets: $\{b, c, s(3)\}$ and $\{b, s(1)\}, \{c, s(2)\}$.
\damiano{spiegare come funziona l'aggregato sopra}
\end{example}

\begin{example}[Choice Rule, Integrity Constraint, and Weak Constraints]
\label{ex:choice_rule_ic_and_wc}
The following logic program extends Example~\ref{ex:choice_rule_and_constraint} with two weak constraints:
\begin{code}
1 {a; b; c} 2.
:- a.
:~ b, not c. [1@1]
:~ c, not b. [1@1]
\end{code}
It admits three answer sets: $\{b, c\}$ and $\{b\}, \{c\}$, whose cost is respectively 0, 1, 1.
Thus, the optimal answer set is $\{b, c\}$. 
\end{example}

% \paragraph{Aggregates} \antonio{\noindent \emph{Aggregates} are set functions over sets of terms. Examples over arithmetic terms are \texttt{\#max}, \texttt{\#sum}, \texttt{\#count}. A formal account of aggregates is beyond the scope of this paper, thus we provide only this intuitive example:}

% \begin{code}
% a(1). a(2). a(3).
% sum(X) :- X = #sum{T: a(T)}.     // sum(6).
% count(X) :- X = #count{T: a(T)}. // count(3).
% max(X) :- X = #max{T: a(T)}.     // max(3).
% min(X) :- X = #max{T: a(T)}.     // max(1).
% \end{code}

% probabilmente omettere e menzionare sotto quando si parla dell'encoding
% \paragraph{\texttt{@}-terms} \antonio{\noindent This feature is not a language extension, but a specific feature of the \textsc{Clingo} system. Other ASP systems support similar features under a different name. \texttt{@}-terms are special terms, whose function name starts with the character \texttt{@} that are replaced with the output of a user-defined procedure upon grounding time. We will use \texttt{@}-terms to perform (fixed precision) floating point arithmetic since ASP does not natively support it.}
%
%

% \subsection{Modeling}
% \antonio{\noindent Finally, the following example shows the standard \emph{Guess \& Check} ASP modeling pattern, where a set of rules (usually positive-cycles normal rules, disjunctive rules or choice rules) are used to generate \emph{candidate solutions}, and integrity constraints are used to \emph{prune} invalid solutions. Although it is common practice to ``split'' encodings into these sections, to ease readability, recall ASP semantics is fully declarative and the order of rules within the program and order of literals within the rules' body does not alter its semantics.}
The modelling procedure adopted in ASP usually is based on \emph{Guess \& Check}: a set of rules (usually a combination of normal rules, disjunctive rules, or choice rules) are used to generate \emph{candidate solutions}, and integrity constraints are used to \emph{prune} invalid solutions.
% Although it is common practice to ``split'' encodings into these sections, to ease readability, recall ASP semantics is fully declarative and the order of rules within the program and order of literals within the rules' body does not alter its semantics.

\begin{example}[Graph Coloring]
\label{ex:running_asp}
Let $G(V,E)$ be an undirected graph over the vertex set $V$ and edge set $E$.
A $k$-coloring is a total function $\lambda: V \mapsto \{1, \dots, k\}$ such that $\lambda(u) \ne \lambda(v)$ for each $\{u,v\} \in E$.
The \emph{graph coloring problem} is the decision problem of computing whether a graph $G$ admits a 3-coloring, and it is well-known to be NP-complete~\cite{aroraComplexity}.
The following answer set program solves the 3-coloring task:
%
\begin{code}
edge(a,b). edge(b,d).
edge(a,c). edge(c,d).
color(red). color(green). color(blue).

node(A):- edge(A,B).
node(B):- edge(A,B).

1 { assign(X,C): color(C) } 1 :- node(X).
:- assign(X,C), assign(Y,C), edge(X,Y).
\end{code}
The $edge/2$ atoms describe the same graph of Example~\ref{ex:running_prolog}.
The three $color/3$ atoms list the available colors (red, green, and blue).
The predicate $node/2$ can be considered as an helper predicate, to extract the nodes involved in the current graph.
The choice rule states that each node must be assigned to exactly one node.
The constraint states that nodes connected by an edge cannot be assigned to the same color.
The considered program has 18 answer sets.

% We encode $G(V,E)$ into a set of facts $F(G) = \{edge(x,y): \{x, y\} \in E\} \cup \{node(x): x \in V\}$.

% The following answer set program solves the 3-coloring task on the answer sets of the following logic program $\Pi$ are in 1-to-1 correspondence with 3-colorings on $G$:

% \noindent $\Pi \cup F(G)$ is incoherent if $G$ is not 3-colorable. If $\Pi \cup F(G)$ is coherent, its answer sets, the atom $assign(x,c)$ is to be interpreted as $\lambda(x) = c$ for each $x \in V$.

As an example of optimization, suppose we wish to find a 3-coloring that uses a given color, say red, as least as possible.
It is sufficient to add these two rules to the previous program to minimize the usage of color red:
\begin{code}
bad_color(red).
:~ bad_color(C), assign(X,C). [1@1,X]
\end{code}
Now, we get 3 optimal answer sets, where the color red is never assigned.
\end{example}




old tabellone
\begin{table}[htb]
\centering
% gloriosa colonna di 0 per i timeout di ASP :heart_eyes:
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Nodes} & \textbf{Images} & \textbf{Failures ASP} & \textbf{Failures Heu.} & \textbf{ASP $<$ 25 s} & \textbf{ASP $<$ 45 s} & \textbf{ASP $>$ 45 s} & \textbf{Heu. $<$ 6 s} & \textbf{Heu. $<$ 12 s} \\ 
\hline
\multirow{3}*{25} & 4 & 0 & 0 & 1000 & 1000 & 0 & 1000 & 1000 \\               
 & 8 & 0 & 0 & 1000 & 1000 & 0 & 1000 & 1000 \\               
 & 12 & 0 & 0 & 992 & 1000 & 0 & 870 & 870 \\
\hline\hline
\multirow{3}*{50} & 4 & 0 & 0 & 1000 & 1000 & 0 & 998 & 1000 \\               
 & 8 & 0 & 1 & 999 & 1000 & 0 & 993 & 998 \\               
 & 12 & 0 & 2 & 966 & 983 & 17 & 864 & 870 \\               
\hline\hline
\multirow{3}*{75} & 4 & 0 & 6 & 1000 & 1000 & 0 & 984 & 991 \\               
 & 8 & 0 & 19 & 987 & 990 & 10 & 957 & 972 \\               
 & 12 & 0 & 22 & 932 & 937 & 63 & 847 & 866 \\ 
\hline\hline
\multirow{3}*{100} & 4 & 0 & 6 & 1000 & 1000 & 0 & 980 & 990 \\               
 & 8 & 0 & 21 & 980 & 983 & 17 & 927 & 953 \\               
 & 12 & 0 & 29 & 838 & 855 & 145 & 787 & 814 \\               
\hline\hline
\multirow{3}*{125} & 4 & 0 & 13 & 1000 & 1000 & 0 & 944 & 963 \\               
 & 8 & 0 & 55 & 966 & 972 & 28 & 855 & 899 \\               
 & 12 & 0 & 71 & 779 & 796 & 204 & 712 & 750 \\               
\hline\hline
\multirow{3}*{150} & 4 & 0 & 24 & 1000 & 1000 & 0 & 923 & 947 \\               
 & 8 & 0 & 81 & 951 & 956 & 44 & 806 & 860 \\               
 & 12 & 0 & 118 & 683 & 715 & 285 & 655 & 704 \\    
\hline
\end{tabular}
\caption{Details of the experiments of Section~\ref{sec:aspvsprolog}. The columns contain, respectively, the number of nodes, images, failures for ASP considered as the number of times ASP cannot find a solution within 60 seconds, failures for iterative deepening considered as the number of times it cannot find a solution within 45 seconds, solutions found with ASP within 25 seconds, solutions found with ASP within 45 seconds, solutions found with ASP with more than 45 seconds, solutions found with iterative deepening within 6 seconds, and solutions found with iterative deepening within 12 seconds over 1000 instances.} 
\end{table}
%\antonio{Recall that our proposed approach works by adapting the image placement by continuous reasoning as long as possible, while computing optimal solutions sparingly when needed (e.g., whenever continuous reasoning fails to find a solution).} \damiano{questa mi sembra una considerazione sull'esperimento 2 mentre la tabella è sul primo esperimento}} % terribile giornata per ASP anche qua :') I failure sono quasi tutti per unsat, devo guardare meglio sì quelli andrebbero scorporati da failures, tenere solo i timeout? concordo, quanto è per asp? è interessante mostrare quanto tempo ci mette a trovare un failure per unsat ASP? credo ci metta meno di prolog, quindi potrebbe essere interessante riportarlo. in questa tabella qua c'è da vedere quanti timeout ("failure vere") rimangono per prolog e asp 
% \caption{Details of the experiments of Section~\ref{sec:aspvsprolog}. The columns contains, respectively, the number of nodes, images, failures for ASP considered as the number of times ASP cannot find a solution within 60 seconds, failures for iterative deepening considered as the number of times it cannot find a solution within 45 seconds, solutions found with ASP within 25 seconds, solutions found with ASP within 45 seconds, solutions found with ASP with more than 45 seconds, solutions found with iterative deepening within 6 seconds, and solutions found with iterative deepening within 12 seconds over 1000 instances. - convince? - convinto, tu questo non lo metteresti?: Recall that our proposed approach attempts to use as much as possible Prolog-based continuous reasoning, while optimal solutions are computed periodically whenever continuous reasoning fails. -- non fa strano due timeout diversi epr due metodi diveris, se il reviewer non è attento?}

% La tabella contiene questo: failures ASP sono ASP timeout (qualsiasi valore) quando soluzione esiste o è unsat, fail heu sono i timeout heu a 45 secondi quando ASP trova la soluzione o dice unsat, le rimanenti colonne sono il numero di soluzioni trovate (per ASP conto anche unsat) entro quel time limit


==> src/preliminaries.tex <==
\section{Background}
\label{sec:preliminaries}

\rev{In this section, we briefly overview some background on Prolog and ASP, needed to understand the content of the next sections.}

\noindent\textbf{\textit{Prolog}}
% 
Prolog is a programming language based on first-order logic~\cite{sterling1994art}. A Prolog program is a set of \textit{rules} (also called \textit{clauses}) of the form:
\begin{code}
h :- b1, ..., bn.
\end{code}
stating that \cd{h} (an atom) holds when the conjunction of literals (i.e., atoms or negated atoms) {\tt b1} $, \dots,$ {\tt bn} ({\tt n}$\geq$0) are all true (i.e., their logical AND holds). 
The atom \cd{h} is called \textit{head} while the conjunction of the literals {\tt bi} is called \textit{body} of the clause. 
% \damiano{Toglierei la frase seguente perché non usiamo regole con digiunzione in testa.}
% \stefano{The logical OR operator $\vee$ can also be used and is denoted as a semi-colon \cd{;} between literals.}

Rules with empty bodies are called \textit{facts} (omitting the \textit{neck} operator, $\impl$). Rules with the same functor (i.e., name and arity) identify a \textit{predicate}.
% , and rules of the same predicate are often referred to as its \textit{clauses}. 
Prolog variables begin with upper-case letters (except for the anonymous variable, which is represented with an underscore, $\_)$, lists are denoted by square brackets and negation by $\backslash +$.
%
We use the standard notation \cd{pred/K} (called functor) to compactly represent a set of atoms or clauses with the atom \cd{pred} as the head and \cd{K} arguments.


\noindent\textbf{\textit{Answer Set Programming}} Answer Set Programming (ASP) is a declarative knowledge representation formalism rooted in the stable model semantics of logic programs~\cite{brewka2011asp}. Despite not being Turing complete, unlike Prolog, ASP has shown to be particularly effective in modelling and solving combinatorial and optimisation problems in a variety of domains. We briefly introduce the typical workflow in ASP applications, recap minimal notions about its syntax and semantics, and provide an example. Interested readers can refer to~\cite{potasscoGuide} for a comprehensive introduction to the ASP language.

ASP requires that a problem instance is encoded into a \emph{logic program} in such a way that its \emph{answer sets} (e.g., its solutions, \emph{models} according to the stable model semantics~\cite{gelfond1988stable}) can be mapped back into solutions of the original program - usually by projecting onto particular predicates. The most common ASP system architecture is based on the \emph{grounding \& solving} approach - where the logic program is first transformed into a propositional one (e.g., one that does not contain variables) which is then passed to a solver component which searches its answer sets.

%We will consider a propositional answer set program, that is a program that does not contain variables. Non-propositional answer set programs (e.g., with variables) can be understood as placeholders for their ``propositional expansion''.
Despite sharing syntactical similarities with Prolog, such as normal rules, atoms, and literals, the semantics of answer set programs is radically different as it relies on the concept of stable models~\cite{gelfond1988stable}.


% An interpretation $\mathcal{I}$ is a set of atoms.
% An interpretation $\mathcal{I}$ \emph{satisfies} a rule $\rho$ if $\mathcal{I} \subseteq B^{+}(\rho)$ and $\mathcal{I} \cap B^{-}(\rho) = \{\}$, where $B^{+}(\rho)$ and $B^{-}(\rho)$ are the set of positive and negative literals in the body of $\rho$, respectively.
% If an interpretation $\mathcal{I}$ satisfies all the rules in $\rho \in P$, $\mathcal{I}$ is a \emph{model} of $P$.
% The \emph{reduct} of $P$ w.r.t. $\mathcal{I}$, denoted as $P^{\mathcal{I}}$, is the logic program we obtain by (i) removing all rules $\rho \in P$ such that $B^{+}(\rho) \not\subseteq \mathcal{I}$ and (ii) removing from the body of each rule $\rho \in P$ the literals $B^{-}(\rho) \cup \mathcal{I}$.
% An interpretation $\mathcal{I}$ is a \emph{stable model} (or \emph{answer set}) of the logic program $P$ if $\mathcal{I}$ is a subset-minimal model of $P^{\mathcal{I}}$.
% ASP semantics is fully declarative and the order of rules within the program and order of literals within the rules' body does not alter it.

%We denote the set of answer sets of a logic program $P$ by $AS(P)$.
%Logic programs under the stable model semantics might admit none, one, or more answer sets. We say that a logic program is \emph{incoherent} if it admits no answer sets, \emph{coherent} otherwise.
%
Modern answer set solvers such as clingo~\cite{gebser2019clingo}, introduce many syntactic shortcuts, which ease the modeling task, such as choice rules, weak constraints, and aggregates. Interested readers can refer to~\cite{potasscoGuide} for a complete reference on the modeling capabilities of the language, and to~\cite{calimeri2012asp} for an up-to-date reference on the language standard.

%\subsubsection{A classic example: Graph Colorability}

%The modelling procedure adopted in ASP usually is based on the \emph{Guess, Check \& Optimise} technique: a set of rules (usually a combination of normal rules, disjunctive rules, or choice rules) are used to generate \emph{candidate solutions}, and integrity constraints are used to \emph{prune} invalid solutions. We showcase the modeling capabilities of ASP by the following example based on the well-known NP-complete Graph Coloring problem.



